Benchmarking and Enhancing Text-to-Image Models for Generating Visual Representations in Early Arithmetic Education

AI systems are increasingly used to support educational content creation, yet it remains unclear whether they can generate outputs that faithfully represent the pedagogical concepts they are intended to teach. Thus, we introduce equation-to-visual generation, a task that, in contrast to conventional image generation, requires producing pedagogically meaningful visuals from arithmetic equations while precisely preserving their numerical and relational structure. Informed by interviews with teachers and an analysis of educational materials, we construct E2V-Bench, a benchmark spanning four pedagogically grounded visual types, along with automatic metrics for evaluating visual correctness. Our evaluation reveals that recent text-to-image (T2I) models frequently fail on this task, with errors dominated by incorrect object counts and broken relational structure. Building on this, we explore benchmark-guided enhancement strategies. These strategies improve representative models, while the remaining gap calls for stronger numerical and relational grounding in future T2I models.

==> sections/06_5_dsl.tex <==


\section{A Structured Reference for E2V}
To better contextualize the low accuracy of current T2I models on E2V-Bench, we further construct a structured rendering pipeline inspired by prior work on template-based educational visual generation~\citep{wang-etal-2025-generating-pedagogically}. Rather than directly generating images from text, this pipeline decomposes the task into two stages: an LLM first maps the \ac{VD} into a domain-specific language (DSL)\footnote{We use GPT-5.4 for DSL generation.}, and a deterministic renderer then converts the DSL into the final visual by editing and arranging icons. This setting is not intended as a directly comparable \ac{T2I} baseline; instead, it serves as a controlled reference for understanding how much of the difficulty arises from image generation versus from the need to preserve precise arithmetic structure. More details of our DSL-based generation pipeline is shown in App.\ref{app:dsl-gen}.

Using this pipeline, we obtain 98.33\% quantity accuracy and 98.33\% overall accuracy for both realistic and cartoon visuals. The remaining errors mainly stem from upstream DSL-generation errors and occasional failures of our automatic metric to correctly recognize rendered icons. These results suggest that the E2V task itself is highly solvable when the required structure is made explicit, and that the main bottleneck for current T2I models lies in faithfully realizing precise numerical and relational constraints in the generated image.
At the same time, this structured pipeline has clear limitations. It relies on a hand-designed DSL, manually collected icon assets, and predefined rendering logic, which restrict flexibility, scalability, and visual diversity. We therefore view it as a diagnostic reference rather than a general solution: it helps explain why current \ac{T2I} models underperform on E2V-Bench, while also highlighting the need for more flexible generative models that can match the faithfulness of structured rendering without relying on manually specified programs.

==> tables/old/table1.tex <==
\begin{table*}
\centering
\scalebox{0.71}{
\begin{tabular}{p{3cm}p{5cm}|cccc}
\toprule
\textbf{Category} & \textbf{Model} & 
\multicolumn{2}{c}{\textbf{Quantity Acc. (\%)}} & 
\multicolumn{2}{c}{\textbf{Overall Acc. (\%)}} \\
 &  & 
\textbf{Realistic} & \textbf{Cartoon} & 
\textbf{Realistic} & \textbf{Cartoon} \\
\midrule
DSL-based
& DSL-based method (ours)
& $\mathbf{98.3 \pm 1.4}$ & $\mathbf{98.3 \pm 1.5}$ & $\mathbf{98.3 \pm 1.4}$ & $\mathbf{98.3 \pm 1.5}$ \\
\midrule
Closed-source   
& Recraft-v3~\citep{recraftv3}   
& $6.0 \pm 2.7$ & $5.7 \pm 2.6$ & $4.7 \pm 2.4$ & $2.7 \pm 1.8$ \\
& GPT-Image-1~\citep{image-1}  
& $27.0 \pm 5.0$ & $22.3 \pm 4.7$ & $21.3 \pm 4.6$ & $17.0 \pm 4.2$ \\
\midrule
Diffusion-based 
& SD-3.5-large~\citep{esser2024scaling} 
& $6.7 \pm 2.9$ & $8.3 \pm 3.1$ & $3.3 \pm 2.1$ & $5.0 \pm 2.5$ \\
& Flux.1-dev~\citep{FLUX1dev}   
& $8.7 \pm 3.2$ & $9.3 \pm 3.3$ & $6.3 \pm 2.8$ & $5.7 \pm 2.6$ \\
\midrule
Layout-to-image 
& Blueprint~\citep{gani2024llm}    
& $2.7 \pm 1.8$ & $1.3 \pm 1.3$ & $1.3 \pm 1.3$ & $1.0 \pm 1.1$ \\
& LMD~\citep{lian2024llmgrounded}          
& $22.4 \pm 4.8$ & $15.3 \pm 4.1$ & $12.0 \pm 3.7$ & $9.7 \pm 3.4$ \\
\midrule
Transformer-based 
& Show-o2~\citep{xie2025show}      
& $4.3 \pm 2.3$ & $4.3 \pm 2.3$ & $2.3 \pm 1.7$ & $3.0 \pm 1.9$ \\
& Bagel~\citep{deng2025bagel}        
& $8.0 \pm 3.1$ & $11.0 \pm 3.6$ & $5.7 \pm 2.6$ & $8.0 \pm 3.1$ \\
\midrule
Prompt refinement 
& PAE~\citep{mo2024dynamic}          
& $1.0 \pm 1.1$ & $3.0 \pm 1.9$ & $1.0 \pm 1.1$ & $1.0 \pm 1.1$ \\
\bottomrule
\end{tabular}
}
\caption{Evaluation of T2I models on E2V-Bench. We report results for both realistic-style and cartoon-style outputs, with 95\% confidence interval half-widths. SD-3.5-large denotes the Stable Diffusion-3.5-large.}
\label{tab:tab1}
\vspace{-5pt}
\end{table*}

==> tables/old/table10.tex <==
\begin{table*}
% \centering
\small
\begin{tabular}{p{2cm}|M{1.5cm}|M{3.5cm}|M{4cm}|M{2cm}}
\hline
\textbf{Dataset} & \textbf{Visuals} & \textbf{Domain} & \textbf{Use Cases} & \textbf{Grade Level} \\
\hline
\sys{} (ours) & 1,903  & Primary School Math Word Problems & 
Supporting primary school students' math understanding; Evaluating and training Text-to-Image models on pedagogical visual generation & Primary school grade 1-3 \\
\hline
MATH-Vision~\citep{wang2024measuring} & 3,040  & General mathematics, competition-level problems & 
Visual math problem-solving; Evaluating multimodal models on math reasoning & Middle school to high school (competition-level difficulty) \\
\hline
MathVista~\citep{lu2024mathvista} & 6,141  & Logical, algebraic, and scientific reasoning & 
Math visual question answering; Puzzle-solving ; logical reasoning; Function analysis ; diagram understanding & Varied (elementary to advanced reasoning) \\
\hline
\end{tabular}

\caption{Dataset Statistics}
\label{tab:tab10}
\label{tab:dataset_comparison}
\end{table*}

==> tables/old/table11.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{2.1cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}M{0.9cm}}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{Quantity Err}} & \multicolumn{2}{c}{\textbf{Relation Err}} & \multicolumn{2}{c}{\textbf{Struct Misalign}} & \multicolumn{2}{c}{\textbf{ Miss Visual Items}} & \multicolumn{2}{c}{\textbf{Miss Contex Cues}}\\
\midrule
 & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive}\\
\midrule
ft\_flux.1-dev(F) & 0.72 & 0.74 & 0.85 & \textbf{0.81} & \textbf{0.35} & \textbf{0.23} & \textbf{0.44} & 0.30 & 0.57 & \textbf{0.49} \\
zs\_flux.1-dev(F) & 0.77 & 0.78 & 0.92 & 0.85 & 1.00 & 1.00 & 0.74 & 0.66 & 0.62 & 0.60 \\
recraft-v3(F)    & \textbf{0.41} & \textbf{0.38} & \textbf{0.82} & \textbf{0.81} & 0.64 & 0.94 & \textbf{0.44} & \textbf{0.18} & \textbf{0.35} & 0.50 \\
\bottomrule
\end{tabular}
\caption{Statistical Results for Qualitative Analysis: For each method, 192 visuals (96 Formal and 96 Intuitive) were evaluated, with each score representing the ratio of corresponding error.}
\label{tab:tab11}
\vspace{-10pt}
\end{table*}

==> tables/old/table12.tex <==
\begin{table*}
\scriptsize
\centering
\begin{tabular}{p{3cm}|M{2cm}|M{3cm}|M{2cm}|M{2cm}}
\hline
\textbf{Work} & \textbf{Arithmetic Coverage} & \textbf{Conceptual Coverage} & \textbf{Semantic Granularity}  & \textbf{Problem Depth} \\
\hline
Visual Language (ours) & (+, -, ×, ÷, surplus, >,<) & Transfer, Rate, Comparison, Part-whole, Surplus, Unit Transformation, Multiple Steps & Concepts \& equations & multiple-order MWP\\
\hline
\citep{opedal-etal-2023-world} & (+, -, ×, ÷) & Transfer, Rate, Comparison, Part-whole & World model & first-order MWP \\
\hline
\citep{hosseini2014learning} & (+, -) & Transfer & World model & first-order MWP \\
\hline
\citep{mitra2016learning} & (+, -) & Transfer, Comparison (add), Part-whole & Concepts \& equations & first-order MWP \\
\hline
\citep{roy2018} & (+, -, ×, ÷) & Transfer, Rate, Comparison, Part-whole, Concepts \& equations & Concepts \& equations & multiple-order MWP \\
\hline
\end{tabular}

\caption{Comparison of our Visual Language approach with existing MWP solvers.}
\label{tab:tab12}
\end{table*}

==> tables/old/table1_combine_version.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{2cm}p{2cm}|M{1.4cm}M{1.4cm}|M{1.4cm}M{1.4cm}|M{1.4cm}M{1.4cm}}
\hline
\textbf{Model} & \textbf{Category} & \multicolumn{2}{c}{\textbf{Quantity Acc. (\%)}} & \multicolumn{2}{c}{\textbf{Semantic Align. (\%)}} & \multicolumn{2}{c}{\textbf{Overall Acc. (\%)}} \\
\hline
 &  & \textbf{Realistic} & \textbf{Cartoon} & \textbf{Realistic} & \textbf{Cartoon} & \textbf{Realistic} & \textbf{Cartoon} \\
\hline
GPT-Image-1        & Closed-source      & \textbf{26.00} & \textbf{21.00} & \textbf{68.67} & \textbf{67.33} & \textbf{23.33} & \textbf{17.00} \\
Recraft-v3         &                     & 5.67  & 5.33  & 40.00 & 36.00 & 5.00  & 2.67  \\
\hline
SD-3.5-large   & Diffusion-based     & 5.67  & 7.67  & 28.33 & 31.00 & 2.00  & 4.67  \\
Flux.1-dev         &                     & 8.00  & 8.33  & 38.00 & 29.33 & 4.67  & 6.00  \\
\hline
LMD                & Layout-to-image     & 21.33 & 15.33 & 40.67 & 41.00 & 14.00 & 8.33  \\
Blueprint          &                     & 2.00  & 1.00  & 23.67 & 27.97 & 1.33  & 0.00  \\
\hline
Bagel              & Transformer-based   & 7.67  & 9.33  & 32.00 & 32.67 & 4.67  & 5.00  \\
Show-o2            &                     & 3.67  & 3.67  & 33.67 & 28.67 & 1.67  & 2.33  \\
\hline
PAE                & Prompt refinement   & 1.00  & 2.33  & 18.67 & 22.67 & 0.33  & 0.67  \\
\hline
\hline
\multicolumn{2}{l|}{LMD+Prompt Refine}                & 25.00 & 19.00 & 47.00 & 46.33 & 17.00 & 11.00 \\
\multicolumn{2}{l|}{LMD+Prompt Refine+Regen}          & \textbf{26.67} & \textbf{19.33} & \textbf{47.67} & \textbf{46.67} & \textbf{18.00} & \textbf{12.00} \\
\multicolumn{2}{l|}{Flux.1-dev (Finetuned)}           & 8.33  & --    & 37.67 & --    & 5.00  & --    \\
\multicolumn{2}{l|}{Bagel (Finetuned)}                & 8.00  & --    & 32.67 & --    & 6.33  & --    \\
\hline
\end{tabular}
\caption{Automatic evaluation of equation-to-visual generation across models on VariMath. We report quantity accuracy, semantic alignment, and overall accuracy for both realistic-style and cartoon-style outputs; fine-tuned models are evaluated on realistic only. SD-3.5-large is abbreviation of Stable Diffusion-3.5-large model.}
\label{tab:tab1}
\vspace{-5pt}
\end{table*}

==> tables/old/table2.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{1.8cm}ccc}
     \toprule
      \textbf{Operation}   & \textbf{Clarity} & \textbf{Engagement} & \textbf{Cog Load Opt}\\
      \midrule
      Addition & 5.4  & 6.4 & 5.0\\
      Subtraction & 5.0  & 6.4 & 5.2\\
      Multiplication & \textbf{7.0}  & 6.4 & \textbf{6.0}\\
      Division & 6.4  & \textbf{6.6} & 5.4\\
      Surplus & 6.8  & \textbf{6.6} & 5.8\\
      Comparison & 5.6  & 6.0 & 4.8\\
      UnitTrans & 6.6  & \textbf{6.6} & 5.6\\
      MultiSteps & 6.6  & \textbf{6.6} & 5.8\\
    \midrule
    \end{tabular}
    \caption{Results of exploratory study session 3. They reflect experts' evaluations of the ``Intuitive'' design for different operations. All scores are on a 7-point Likert scale, where higher values indicate better performance.}
    \label{tab:tab2}
\end{table}


==> tables/old/table3.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{5.5cm}p{1cm}}
     \toprule
      \textbf{Criterion}   & \textbf{Score} \\
      \midrule
      Helps in understanding MWP & 6.8\\
      Useful for teaching & \textbf{7.0}\\
      Like to use these visuals frequently & \textbf{7.0} \\
    \midrule
    \end{tabular}
    \caption{Results of post-task questionnaire.\april{The tables and figures should be understandable independent of the text. What does a score of 7.0 mean?}}
    \label{tab:tab3}
\end{table}

==> tables/old/table4.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{3cm}p{1.5cm}p{1.7cm}}
     \toprule
      \textbf{Criterion}   & \textbf{Edit Dist$\downarrow$}  & \textbf{LM Ratio$\uparrow$} \\
      \midrule
     o3-mini(F) & 2.82 & \textbf{96.89}\\
     o3-mini & 2.90 & 91.05\\
      gemini-2-flash(F) & \textbf{2.67} & 90.27\\
      gemini-2-flash & 2.96 & 72.76\\
    \midrule
    ft\_llama-3.1-8B(F) & \textbf{2.28} & \textbf{89.50} \\
    ft\_llama-3.1-8B & 2.52 & 80.54 \\
    zs\_llama-3.1-8B(F) & 4.67 & 1.95 \\
    zs\_llama-3.1-8B & 4.47 & 3.11 \\
    \hline
    \end{tabular}
    \caption{Visual Language Generation Results: F indicates generation with the solution formula. Scores are averaged over 257 \(VL\) instances per method.}
    \label{tab:tab4}
    \vspace{-15pt}
\end{table}

==> tables/old/table5.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{3cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}}
\hline
\textbf{Method} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Completeness}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Cog Load Opt}} \\
\hline
 & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} \\
\hline
o3-mini(F) & \textbf{4.92} & 4.58 & \textbf{5.00} & \textbf{4.67} & 4.88 & 4.67 & \textbf{4.96} & 4.54 \\
o3-mini(NF) & 4.83 & 4.54 & 4.96 & 4.50 & \textbf{5.00} & 4.67 & \textbf{4.96} & 4.42 \\
gemini-2-flash(F) & 4.79 & 4.50 & 4.92 & 4.57 & 4.96 & \textbf{4.79} & \textbf{4.96} & \textbf{4.65} \\
gemini-2-flash(NF) & 4.54 & \textbf{4.62} & 4.58 & 4.57 & 4.79 & 4.67 & 4.75 & 4.61 \\
recraft-v3(F) & 3.33 & 2.96 & 3.75 & 3.62 & 3.75 & 4.00 & 3.63 & 3.96 \\
recraft-v3(NF) & 3.26 & 2.96 & 3.50 & 3.33 & 3.54 & 3.75 & 3.54 & 3.92 \\
dalle-3(F) & 2.96 & 3.04 & 3.21 & 3.42 & 2.54 & 2.33 & 2.54 & 2.50 \\
dalle-3(NF) & 2.79 & 2.96 & 2.83 & 3.33 & 2.12 & 2.29 & 2.17 & 2.46 \\
\midrule
\midrule
ft\_llama-3.1-8B(F)   & \textbf{4.79} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} \\
ft\_llama-3.1-8B(NF)  & 4.58 & \textbf{4.83} & 4.63 & \textbf{4.83} & 4.67 & \textbf{4.83} & 4.67 & \textbf{4.83} \\
zs\_llama-3.1-8B(F)   & 1.25 & 1.33 & 1.25 & 1.33 & 1.33 & 1.33 & 1.29 & 1.33 \\
zs\_llama-3.1-8B(NF)  & 1.08 & 1.00 & 1.04 & 1.00 & 1.17 & 1.00 & 1.17 & 1.00 \\
ft\_flux.1-dev(F)      & 3.21 & 2.62 & 3.38 & 3.38 & 3.38 & 3.12 & 3.50 & 3.33 \\
ft\_flux.1-dev(NF)    & 3.12 & 2.21 & 3.33 & 3.38 & 3.33 & 3.17 & 3.29 & 3.25 \\
zs\_flux.1-dev(F)    & 3.13 & 2.50 & 3.21 & 2.83 & 3.33 & 3.25 & 3.42 & 3.63 \\
zs\_flux.1-dev(NF)   & 3.13 & 2.42 & 3.21 & 2.83 & 3.33 & 3.25 & 3.42 & 3.63 \\
\midrule
\midrule
o3-mini(F)   & \textbf{4.97} & \textbf{4.96} & \textbf{5.00} & \textbf{4.97} & \textbf{4.94} & \textbf{4.94} & \textbf{4.96} & \textbf{4.96} \\
recraft-v3(F)  & 2.65 & 3.00 & 3.57 & 3.82 & 3.58 & 3.76 & 3.18 & 3.29 \\

ft\_llama-3.1-8B(F)   & \textbf{4.93} & \textbf{4.92} & \textbf{4.92} & \textbf{4.92} & \textbf{4.99} & \textbf{4.92} & \textbf{4.96} & \textbf{4.97} \\
ft\_flux.1-dev(F)  & 2.49 & 2.53 & 2.60 & 2.64 & 3.67 & 3.54 & 3.89 & 3.92 \\
\hline
\end{tabular}
\caption{Human Evaluation of Visual Representations. In the upper and middle parts, 48 visuals (24 Formal, 24 Intuitive) were evaluated with scores averaged from two researchers on a 1–5 scale. In the lower part, 144 visuals (72 Formal, 72 Intuitive) were evaluated. (F) indicates use of the solution formula as input, while (NF) indicates otherwise; “ft” denotes a fine-tuned model and “zs” a zero-shot model.}
\label{tab:tab5}
\vspace{-5pt}
\end{table*}

==> tables/old/table5_redesign.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{.1cm}p{2cm}M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}M{1cm}}
\toprule
& \textbf{Method} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Completeness}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Cog Load Opt}} \\
\midrule
& & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} \\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{prompting}} 
& o3-mini(F) & \textbf{4.92} & 4.58 & \textbf{5.00} & \textbf{4.67} & 4.88 & 4.67 & \textbf{4.96} & 4.54 \\
& o3-mini & 4.83 & 4.54 & 4.96 & 4.50 & \textbf{5.00} & 4.67 & \textbf{4.96} & 4.42 \\
& gemini-2-flash(F) & 4.79 & 4.50 & 4.92 & 4.57 & 4.96 & \textbf{4.79} & \textbf{4.96} & \textbf{4.65} \\
& gemini-2-flash & 4.54 & \textbf{4.62} & 4.58 & 4.57 & 4.79 & 4.67 & 4.75 & 4.61 \\
& recraft-v3(F) & 3.33 & 2.96 & 3.75 & 3.62 & 3.75 & 4.00 & 3.63 & 3.96 \\
& recraft-v3 & 3.26 & 2.96 & 3.50 & 3.33 & 3.54 & 3.75 & 3.54 & 3.92 \\
& dalle-3(F) & 2.96 & 3.04 & 3.21 & 3.42 & 2.54 & 2.33 & 2.54 & 2.50 \\
& dalle-3 & 2.79 & 2.96 & 2.83 & 3.33 & 2.12 & 2.29 & 2.17 & 2.46 \\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{fine-tuning}} 
&
ft\_llama-3.1-8B(F)   & \textbf{4.79} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} & \textbf{4.83} \\
& ft\_llama-3.1-8B  & 4.58 & \textbf{4.83} & 4.63 & \textbf{4.83} & 4.67 & \textbf{4.83} & 4.67 & \textbf{4.83} \\
& zs\_llama-3.1-8B(F)   & 1.25 & 1.33 & 1.25 & 1.33 & 1.33 & 1.33 & 1.29 & 1.33 \\
& zs\_llama-3.1-8B  & 1.08 & 1.00 & 1.04 & 1.00 & 1.17 & 1.00 & 1.17 & 1.00 \\
& ft\_flux.1-dev(F)      & 3.21 & 2.62 & 3.38 & 3.38 & 3.38 & 3.12 & 3.50 & 3.33 \\
& ft\_flux.1-dev    & 3.12 & 2.21 & 3.33 & 3.38 & 3.33 & 3.17 & 3.29 & 3.25 \\
& zs\_flux.1-dev(F)    & 3.13 & 2.50 & 3.21 & 2.83 & 3.33 & 3.25 & 3.42 & 3.63 \\
& zs\_flux.1-dev   & 3.13 & 2.42 & 3.21 & 2.83 & 3.33 & 3.25 & 3.42 & 3.63 \\
\midrule\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{exp. eval}} 
 & o3-mini(F)   & \textbf{4.97} & \textbf{4.96} & \textbf{5.00} & \textbf{4.97} & 4.94 & \textbf{4.94} & \textbf{4.96} & 4.96 \\
& recraft-v3(F)  & 2.65 & 3.00 & 3.57 & 3.82 & 3.58 & 3.76 & 3.18 & 3.29 \\

& ft\_llama-3.1-8B(F)   & 4.93 & 4.92 & 4.92 & 4.92 & \textbf{4.99} & 4.92 & \textbf{4.96} & \textbf{4.97} \\
& ft\_flux.1-dev(F)  & 2.49 & 2.53 & 2.60 & 2.64 & 3.67 & 3.54 & 3.89 & 3.92 \\
\bottomrule
\end{tabular}
\caption{Human Evaluation of Visual Representations: In the upper and middle parts of the table, 48 visuals (24 Formal, 24 Intuitive) were evaluated with scores averaged from two researchers on a 1–5 scale. In the lower part (expanded evaluation), 144 visuals (72 Formal, 72 Intuitive) were further evaluated with the best performing models. (F) indicates use of the solution formula as input; “ft” denotes a fine-tuned model and “zs” a zero-shot model.}
\label{tab:tab5}
\vspace{-5pt}
\end{table*}

==> tables/old/table6.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{3cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}}
\hline
\textbf{Method} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Completeness}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Cog Load Opt}} \\
\hline
 & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} \\
\hline
o3-mini(F)   & \textbf{4.97} & \textbf{4.96} & \textbf{5.00} & \textbf{4.97} & \textbf{4.94} & \textbf{4.94} & \textbf{4.96} & \textbf{4.96} \\
recraft-v3(F)  & 2.65 & 3.00 & 3.57 & 3.82 & 3.58 & 3.76 & 3.18 & 3.29 \\
\midrule
\midrule
ft\_llama-3.1-8B(F)   & \textbf{4.93} & \textbf{4.92} & \textbf{4.92} & \textbf{4.92} & \textbf{4.99} & \textbf{4.92} & \textbf{4.96} & \textbf{4.97} \\
ft\_flux.1-dev(F)  & 2.49 & 2.53 & 2.60 & 2.64 & 3.67 & 3.54 & 3.89 & 3.92 \\
\hline
\end{tabular}

\caption{Expanded Human Evaluation of Selected Models: For each method, 144 visuals (72 Formal and 72 Intuitive) were evaluated. Each score is the average of two researchers' ratings on a 1–5 scale (higher is better).}
\label{tab:tab6}
\vspace{-10pt}
\end{table*}

==> tables/old/table7.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{cp{2cm}p{1cm}p{2cm}}
     \toprule
      \textbf{PID}   & \textbf{Language in Teaching} & \textbf{Age} & \textbf{Gender}\\
      \midrule
      
       1 & English  & 52 & Male\\
       2 & English  & 45 & Male\\
       3 & English  & 35 & Female\\
       4 & English  & 44 & Female\\
       5 & English  & 37 & Female\\
       

      \bottomrule       
    \end{tabular}
    \caption{Participants' Demographics: We recruited five primary school math teachers who teach grades 1–3 through Prolific. All teachers consider themselves experienced educators in using visuals to teach MWPs.}
    \label{tab:tab7}
\end{table}


==> tables/old/table8.tex <==
\begin{table*}
\centering
\scriptsize
\begin{tabular}{p{4.3cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}|M{1cm}M{1cm}}
\hline
\textbf{Method} & \multicolumn{2}{c}{\textbf{Accuracy}} & \multicolumn{2}{c}{\textbf{Completeness}} & \multicolumn{2}{c}{\textbf{Clarity}} & \multicolumn{2}{c}{\textbf{Cog Load Opt}} \\
\hline
 & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} & \textbf{Formal} & \textbf{Intuitive} \\
\hline
ft\_ mistral-7B-v0.3(F) & 2.83 & 2.71 & 3.00 & 2.67 & \textbf{3.00} & 2.71 & \textbf{2.96} & 2.71 \\
ft\_ mistral-7B-v0.3(NF)  & 2.54 & 2.08 & 2.67 & 2.04 & 2.67  & 2.08 & 2.63 & 2.08 \\
zs\_ mistral-7B-v0.3(F) & 1.33 & 1.00 & 1.38 & 1.00 & 1.46  & 1.00 & 1.46 & 1.00 \\
zs\_ mistral-7B-v0.3(NF)  & 1.25 & 1.00 & 1.21 & 1.00 & 1.29  & 1.00 & 1.33 & 1.00 \\
ft\_stable-diffusion-3.5-large(F)  & \textbf{2.96} & \textbf{2.88} & \textbf{3.12} & \textbf{3.08} & 2.92 & \textbf{3.75} & 2.83 & \textbf{3.58} \\
ft\_stable-diffusion-3.5-large(NF) & \textbf{2.96} & 2.75 & 3.08 & \textbf{3.08} & 2.79 & 3.58 & 2.83 & 3.54 \\
zs\_stable-diffusion-3.5-large(F)  & 2.71 & 2.67 & 2.96 & 2.92 & 2.83 & 3.08 & 2.83 & 2.96 \\
zs\_stable-diffusion-3.5-large(NF) & 2.71 & 2.67 & 2.96 & 2.71 & 2.83 & 3.08 & 2.83 & 2.96 \\
\hline
\end{tabular}
\caption{Other evaluation results for different visual generation methods. For each method, 48 visuals (24 Formal and 24 Intuitive) were evaluated, with each score representing the average rating from two researchers on a 1–5 scale (higher is better).  (F) indicates the method used the solution formula as input, while (NF) indicates it did not. ``ft'' means this model is fine-tuned on our annotated dataset, while ``zs'' means zero-shot.}
\label{tab:tab8}
\end{table*}

==> tables/old/table9.tex <==
\begin{table}[h]
    \centering
    \small
    \begin{tabular}{p{3.2cm}p{1.5cm}p{1.7cm}}
     \toprule
      \textbf{Criterion}   & \textbf{Edit Dist$\downarrow$}  & \textbf{LM Ratio$\uparrow$} \\
      \midrule
    ft\_ mistral-7B-v0.3(F) & \textbf{2.98} & \textbf{39.30} \\
    ft\_ mistral-7B-v0.3(NF) & 3.14 & 19.07 \\
    zs\_ mistral-7B-v0.3(F) & 7.05 & 0 \\
    zs\_ mistral-7B-v0.3(NF) & 6.86 & 0 \\
    \hline
    \end{tabular}
    \caption{Other results of Visual Language generation. F denotes generation with the solution formula as input, while NF denotes generation without the formula.}
    \label{tab:tab9}
\end{table}

==> tables/old/temp.tex <==
ft\_flux.1-dev(F) & 69 & 71 & 82 & 78 & 34 & 22 & 42 & 29 & 80 & 77 \\
zs\_flux.1-dev(F) & 74 & 75 & 88 & 82 & 96 & 96 & 71 & 63 & 89 & 95 \\
recraft-v3(F) & 39 & 36 & 79 & 78 & 147 & 105 & 42 & 17 & 56 & 84 \\
\text

==> tables/table11.tex <==
% \begin{table}[h]
% \centering
% \scriptsize
% \begin{tabular}{lccc}
% \toprule
% \textbf{Quantity Range} & \textbf{Group Share (\%)} & \textbf{Realistic StyleOverall Accuracy (\%)} & \textbf{Cartoon Style Overall Accuracy (\%)} \\
% \midrule
% 1--5   & 18.67 & 15.87 & 11.51 \\
% 6--10  & 33.33 & 6.56 & 5.44 \\
% 11--15 & 29.00 & 2.81 & 2.68 \\
% 16--20 & 19.00 & 1.95 & 2.34 \\
% \bottomrule
% \end{tabular}
% \caption{Overall accuracy across object quantity ranges, together with the proportion of examples each range covers in the dataset.}
% \label{tab:tab11}
% \end{table}

\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Quantity Range} & \textbf{Group Share (\%)} &
\makecell{\textbf{Realistic Style}\\\textbf{Overall Accuracy (\%)}} &
\makecell{\textbf{Cartoon Style}\\\textbf{Overall Accuracy (\%)}} \\
\midrule
1--5   & 18.67 & 15.87 & 11.51 \\
6--10  & 33.33 &  6.56 &  5.44 \\
11--15 & 29.00 &  2.81 &  2.68 \\
16--20 & 19.00 &  1.95 &  2.34 \\
\bottomrule
\end{tabular}
\caption{Overall accuracy across object quantity ranges, together with the proportion of examples each range covers in the dataset.}
\label{tab:tab11}
\end{table}




==> tables/table12.tex <==
% \begin{table}[h]
% \centering
% \scriptsize
% \begin{tabular}{lccc}
% \toprule
% \textbf{Visual Type} & \textbf{Group Share (\%)} & \textbf{Realistic Style Overall Accuracy (\%)} & \textbf{Cartoon Style Overall Accuracy (\%)} \\
% \midrule
% Color     & 25.00 & 8.74 & 6.07 \\
% Object    & 25.00 & 7.41 & 6.52 \\
% Spatial  & 25.00 & 7.56 & 5.93 \\
% Container & 25.00 & 1.63 & 2.22 \\
% \bottomrule
% \end{tabular}
% \caption{Overall accuracy across visual types, together with the proportion of examples each type covers in the dataset.}
% \label{tab:tab12}
% \end{table}


\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{lccc}
\toprule
\textbf{Visual Type} & \textbf{Group Share (\%)} &
\makecell{\textbf{Realistic Style}\\\textbf{Overall Accuracy (\%)}} &
\makecell{\textbf{Cartoon Style}\\\textbf{Overall Accuracy (\%)}} \\
\midrule
Color     & 25.00 & 8.74 & 6.07 \\
Object    & 25.00 & 7.41 & 6.52 \\
Spatial   & 25.00 & 7.56 & 5.93 \\
Container & 25.00 & 1.63 & 2.22 \\
\bottomrule
\end{tabular}
\caption{Overall accuracy across visual types, together with the proportion of examples each type covers in the dataset.}
\label{tab:tab12}
\end{table}

==> tables/table13.tex <==
\begin{table}[h]

\centering
\scriptsize
\begin{tabular}{llccc}
\toprule
\textbf{Operation} & \textbf{Quantity Range} & \textbf{Group Share (\%)} & \textbf{Realistic Style Accuracy (\%)} & \textbf{Cartoon Style Accuracy (\%)} \\
\midrule
Addition       & 1--5   & 0.00  & --    & --    \\
               & 6--10  & 25.00 & 2.78  & 3.89  \\
               & 11--15 & 50.00 & 2.50  & 1.94  \\
               & 16--20 & 25.00 & 0.56  & 1.67  \\
\midrule
Division       & 1--5   & 30.00 & 12.96 & 14.81 \\
               & 6--10  & 10.00 & 2.78  & 0.00  \\
               & 11--15 & 47.50 & 2.92  & 2.34  \\
               & 16--20 & 12.50 & 0.00  & 0.00  \\
\midrule
Multiplication & 1--5   & 0.00  & --    & --    \\
               & 6--10  & 42.86 & 8.33  & 5.56  \\
               & 11--15 & 14.29 & 8.33  & 5.56  \\
               & 16--20 & 42.86 & 3.70  & 2.78  \\
\midrule
Subtraction    & 1--5   & 28.95 & 14.90 & 10.61 \\
               & 6--10  & 42.11 & 7.12  & 6.25  \\
               & 11--15 & 15.79 & 1.85  & 2.78  \\
               & 16--20 & 13.16 & 2.22  & 3.33  \\
\bottomrule
\end{tabular}
\caption{Accuracy across operations and object quantity ranges, together with the proportion of examples each range covers in the dataset.}
\label{tab:tab13}
\end{table}

==> tables/table18.tex <==
% \begin{table}[t]
% \centering
% \scalebox{0.65}{
% \setlength{\tabcolsep}{3pt} % tighten column spacing
% \begin{tabular}{lccc}
% \toprule
% \textbf{Method} 
% & \textbf{Quant. Acc. (\%)} 
% & \textbf{Overall Acc. (\%)}  \\
% \midrule
% GPT-Image-1 
% & 29.67  & \textbf{27.47}  \\
% LMD (PR+Regen)                  
% & \textbf{30.77}  & 20.33   \\
% Bagel (RSFT)
% & 20.88 & \textbf{19.23}  \\
% \bottomrule
% \end{tabular}
% }
% \caption{Human evaluation of the performance of three models on a real educational visual dataset.}
% \label{tab:tab18}
% \vspace{-15pt}
% \end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/source/fig4_rev.pdf}
    \caption{Human evaluation of the performance of three models on a real educational visual dataset.}
    \label{tab:tab18}
    \vspace{-15pt}
\end{figure}

==> tables/table19_clipscore.tex <==
\begin{table*}
\centering
\scalebox{0.71}{
\begin{tabular}{p{3cm}p{5cm}|
cc}
\toprule
\textbf{Category} & \textbf{Model} & 
\multicolumn{2}{c}{\textbf{CLIPScore}} \\
 &  & 
\textbf{Realistic} & \textbf{Cartoon} \\
\midrule
Closed-source   
& Recraft-v3~\citep{recraftv3}   
& 0.81 & 0.78 \\
& GPT-Image-1~\citep{image-1}  
& 0.80 & 0.81 \\
\midrule
Diffusion-based 
& SD-3.5-large~\citep{esser2024scaling} 
& 0.80 & 0.80 \\
& Flux.1-dev~\citep{FLUX1dev}   
& 0.77 & 0.75 \\
\midrule
Layout-to-image 
& Blueprint~\citep{gani2024llm}    
& 0.74 & 0.73 \\
& LMD~\citep{lian2024llmgrounded}          
& 0.75 & 0.71 \\
\midrule
Transformer-based 
& Show-o2~\citep{xie2025show}      
& \textbf{0.82} & \textbf{0.82} \\
& Bagel~\citep{deng2025bagel}        
& 0.77 & 0.79 \\
\midrule
Prompt refinement 
& PAE~\citep{mo2024dynamic}          
& 0.70 & 0.69 \\
\midrule
\textbf{Refined models} 
& LMD                       
& 0.75 & -- \\
& LMD+PR                   
& 0.76 & -- \\
& LMD (PR+Regen)             
& \textbf{0.76} & -- \\
\midrule
& Flux.1-dev               
& 0.77 & -- \\
& Flux.1-dev (SFT)         
& \textbf{0.78} & -- \\
\midrule
& Bagel                    
& 0.77 & -- \\
& Bagel (SFT)              
& \textbf{0.78} & -- \\
\bottomrule
\end{tabular}
}
\caption{CLIPScore of T2I models on \ac{E2V-Bench}. Refined models are evaluated on realistic-style visual generation only.}
\label{tab:tab_clipscore}
\vspace{-5pt}
\end{table*}

==> tables/table2.tex <==
\begin{table}[h]
    \centering
    \caption{Cohen's kappa agreement between human annotations and automatic metrics across different evaluation criteria.}
    \small
    \begin{tabular}{p{3cm}p{2.5cm}}
     \toprule
      \textbf{Criterion}   & \textbf{Cohen's kappa} \\
      \midrule
      Overall Accuracy   & 0.85 \\
      Quantity Accuracy  & 0.74 \\
      Semantic Alignment  & 0.76 \\
    \midrule
    \end{tabular}
    \label{tab:tab2}
    \vspace{-10pt}
\end{table}

==> tables/table4.tex <==
\begin{table}[t]
\centering
\scalebox{0.66}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
\textbf{Method} 
& \textbf{Quant. Acc. (\%)} 
& \textbf{Overall Acc. (\%)} \\
\midrule
LMD 
& $22.4 \pm 4.8$ & $12.0 \pm 3.7$ \\
\rowcolor{hj_gray!30}LMD+PR              
& $26.7 \pm 5.1$ & $14.7 \pm 4.1$ \\
\rowcolor{hj_gray!70}LMD (PR+Regen)        
& $\mathbf{26.7 \pm 5.0}$ & $\mathbf{15.3 \pm 4.1}$ \\
\midrule
Flux.1-dev        
& $\mathbf{8.7 \pm 3.2}$ & $\mathbf{6.3 \pm 2.8}$ \\
\rowcolor{hj_gray!30}Flux.1-dev (SFT)         
& $8.0 \pm 3.1$ & $5.3 \pm 2.6$ \\
\midrule
Bagel              
& $\mathbf{8.0 \pm 3.1}$ & $5.7 \pm 2.6$ \\
\rowcolor{hj_gray!30}Bagel (SFT)              
& $\mathbf{8.0 \pm 3.1}$ & $\mathbf{6.3 \pm 2.8}$ \\
\bottomrule
\end{tabular}
}
\caption{Evaluation of refined models on realistic-style visual generation. PR means prompt refinement, and Regen means regeneration. Values are shown as accuracy with 95\% confidence interval half-widths.}
\label{tab:tab4}
\vspace{-12pt}
\end{table}


% lmd_realistic_mwp_prompt_refine_formulation_eval.csv | quantity_accuracy: 26.67 ± 5.06 (21.61, 31.73), n=300
% lmd_realistic_mwp_prompt_refine_formulation_eval.csv | final_accuracy: 14.67 ± 4.05 (10.62, 18.71), n=300

% \begin{table}[t]
% \centering
% \scalebox{0.66}{
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Method} 
% & \textbf{Quant. Acc. (\%)} 
% & \textbf{Overall Acc. (\%)} \\
% \midrule
% LMD 
% & 22.3 [18.1, 27.5] & 12.0 [8.8, 16.2] \\
% \rowcolor{hj_gray!30}LMD+PR              
% & \textbf{26.7} [22.0, 31.9] & 14.7 [11.1, 19.1] \\
% \rowcolor{hj_gray!70}LMD (PR+Regen)        
% & \textbf{26.7} [22.0, 31.9] & \textbf{15.3} [11.7, 19.9] \\
% \midrule
% Flux.1-dev        
% & \textbf{8.7} [6.0, 12.4] & \textbf{6.3} [4.1, 9.7] \\
% \rowcolor{hj_gray!30}Flux.1-dev (SFT)         
% & 8.0 [5.4, 11.6] & 5.3 [3.3, 8.5] \\
% \midrule
% Bagel              
% & 8.0 [5.4, 11.6] & 5.7 [3.6, 8.9] \\
% \rowcolor{hj_gray!30}Bagel (SFT)              
% & 8.0 [5.4, 11.6] & 6.3 [4.1, 9.7] \\
% \bottomrule
% \end{tabular}
% }
% \caption{Evaluation of refined models on realistic-style visual generation. PR means prompt refinement, and Regen means regeneration. Values are percentages; brackets indicate 95\% Wilson confidence intervals.}
% \label{tab:tab4}
% \vspace{-12pt}
% \end{table}

==> tables/table4_old.tex <==
\begin{table}[t]
\centering
\scalebox{0.66}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
\textbf{Method} 
& \textbf{Quant. Acc. (\%)} 
& \textbf{Overall Acc. (\%)} \\
\midrule
LMD 
& 22.3 & 12.0 \\
\rowcolor{hj_gray!30}LMD+PR              
& \textbf{26.7} & 14.7 \\
\rowcolor{hj_gray!70}LMD (PR+Regen)        
& \textbf{26.7} & \textbf{15.3} \\
\midrule
Flux.1-dev        
& \textbf{8.7} & \textbf{6.3} \\
\rowcolor{hj_gray!30}Flux.1-dev (SFT)         
& 8.0 & 5.3 \\
\midrule
Bagel              
& 8.0 & 5.7 \\
\rowcolor{hj_gray!30}Bagel (SFT)              
& 9.0 & 6.0 \\
\bottomrule
\end{tabular}
}
\caption{Evaluation of refined models on realistic-style visual generation. PR means with prompt refinement and Regen means with regeneration.}
\label{tab:tab4}
\vspace{-12pt}
\end{table}
